Rates of tidal disruption of stars by massive central black holes

There is strong evidence for some kind of massive dark object in the centres of many galaxy bulges. The detection of flares from tidally disrupted stars could confirm that these objects are black holes (BHs). Here we present calculations of the stellar disruption rates in detailed dynamical models of real galaxies, taking into account the refilling of the loss cone of stars on disruptable orbits by two-body relaxation and tidal forces in non-spherical galaxies. The highest disruption rates (one star per 10^4 yr) occur in faint (L>10^10 L_sun) galaxies, which have steep central density cusps. More luminous galaxies are less dense and have much longer relaxation times and more massive BHs. Dwarf stars in such galaxies are swallowed whole by the BH and hence do not emit flares; giant stars could produce flares as often as every 10^5 yr, although the rate depends sensitively on the shape of the stellar distribution function. We discuss the possibility of detecting disruption flares in current supernova searches. The total mass of stars consumed over the lifetime of the galaxy is of order 10^6 M_sun, independent of galaxy luminosity; thus disrupted stars may contribute significantly to the present BH mass in galaxies fainter than about 10^9 L_sun.

==> table.tex <==
\input mn
\landscape
\authorcomment{Landscape Table to be pasted into the article.}
\begintopmatter
\maketitle
\def\yr{{\rm\,yr}}
\begintable{1}
\caption{{\bf Table 1.} Fuelling Rates}
\halign{\bf #\hfil &\quad %% Galaxy name
  \hfil# &\quad %% Type
  \hfil# &\quad %% Distance
  \hfil# &\quad %% Luminosity
  \hfil# &\quad %% M/L
  \hfil# &\quad %% M_bh
  \hfil# &\quad %% r_h
  \qquad
  \hfil# &\quad %% Flux(2body,solar)
  \hfil# &\quad %% Flux(2body,MF)
  \hfil# &\quad %% Flux(total,solar)
  \hfil# &\quad %% Flux(total,MF)
  \hfil#\cr %% logrmean
Galaxy & Type & $D$/Mpc & 
  $\log \left(L_V\over L_\odot\right)$ & 
  $\Upsilon_V/\Upsilon_\odot$ & 
  $\log \left(M_\bullet \over M_\odot\right)$ & 
  $r_{\rm h}$/arcsec & 
  $\log (F^{\rm lc}_\odot/\yr^{-1})$ & 
  $\log (F^{\rm lc}_{\rm MF}/\yr^{-1})$ & 
  $\log (F_\odot/\yr^{-1})$ & 
  $\log (F_{\rm MF}/\yr^{-1})$ &
  $\log(r_{\rm apo}/{\rm arcsec})$\cr
\noalign{\vskip3pt\hrule\vskip3pt}
       M31 & S$\cap$ &    0.8 &    9.860&
     4.8 &    7.792 &     4.19 &
$   -5.18\pm    0.11$ & $   -6.23\pm    0.12$ &
 $   -5.06\pm    0.08$ & $   -4.68\pm    0.07$ & $  1.90\pm  0.35$\cr
       M32 & E$\setminus$ &    0.8 &    8.572&
     2.2 &    6.376 &     0.33 &
$   -4.15\pm    0.10$ & $   -3.91\pm    0.11$ &
 $   -3.91\pm    0.02$ & $   -3.62\pm    0.02$ & $ -0.40\pm  0.48$\cr
   NGC~821 & E$\setminus$ &   19.5 &   10.188&
     8.3 &    8.298 &     0.17 &
$   -4.79\pm    0.13$ & $   -7.20\pm    0.13$ &
 $   -4.48\pm    0.08$ & $   -5.18\pm    0.09$ & $  0.49\pm  0.41$\cr
  NGC~1399 & E$\cap$ &   17.9 &   10.616&
     7.8 &    9.718 &     2.57 &
$   -5.29\pm    0.20$ & $   -7.72\pm    0.20$ &
 $   -3.92\pm    0.34$ & $   -4.51\pm    0.34$ & $  1.09\pm  0.28$\cr
\noalign{\vskip3pt}
  NGC~1600 & E$\cap$ &   50.2 &   11.012&
    12.1 &   10.059 &     1.61 &
$   -6.12\pm    0.09$ & $   -8.55\pm    0.09$ &
 $   -3.84\pm    0.04$ & $   -4.43\pm    0.04$ & $  0.75\pm  0.18$\cr
  NGC~2300 & E$\cap$ &   31.8 &   10.660&
     8.8 &    9.454 &     1.13 &
$   -5.66\pm    0.09$ & $   -8.09\pm    0.09$ &
 $   -4.34\pm    0.06$ & $   -4.93\pm    0.06$ & $  0.71\pm  0.27$\cr
  NGC~2832 & E$\cap$ &   90.2 &   11.112&
     7.6 &   10.058 &     0.97 &
$   -5.86\pm    0.09$ & $   -8.30\pm    0.09$ &
 $   -3.92\pm    0.10$ & $   -4.51\pm    0.10$ & $  0.48\pm  0.24$\cr
  NGC~3115 & S0$\setminus$ &    8.4 &   10.232&
     8.0 &    8.608 &     0.35 &
$   -4.24\pm    0.08$ & $   -6.64\pm    0.08$ &
 $   -3.95\pm    0.05$ & $   -5.30\pm    0.05$ & $  0.80\pm  0.50$\cr
\noalign{\vskip3pt}
  NGC~3377 & E$\setminus$ &    9.9 &    9.812&
     2.8 &    7.786 &     0.14 &
$   -4.19\pm    0.66$ & $   -4.98\pm    0.26$ &
 $   -3.94\pm    0.30$ & $   -4.48\pm    0.13$ & $ -0.41\pm  0.84$\cr
  NGC~3379 & E$\cap$ &    9.9 &   10.152&
     5.3 &    8.594 &     0.56 &
$   -5.07\pm    0.13$ & $   -7.49\pm    0.13$ &
 $   -4.88\pm    0.06$ & $   -5.32\pm    0.07$ & $  1.06\pm  0.30$\cr
  NGC~3608 & E$\cap$ &   20.3 &   10.268&
     5.9 &    8.392 &     0.23 &
$   -4.88\pm    0.02$ & $   -7.29\pm    0.02$ &
 $   -4.67\pm    0.15$ & $   -5.13\pm    0.07$ & $  0.63\pm  0.31$\cr
  NGC~4168 & E$\cap$ &   36.4 &   10.636&
     5.9 &    9.077 &     0.68 &
$   -5.94\pm    0.17$ & $   -8.36\pm    0.18$ &
 $   -4.84\pm    0.05$ & $   -5.36\pm    0.04$ & $  0.59\pm  0.29$\cr
\noalign{\vskip3pt}
  NGC~4278 & E$\cap$ &   17.5 &   10.396&
     5.7 &    9.166 &     1.24 &
$   -5.34\pm    0.05$ & $   -7.76\pm    0.05$ &
 $   -4.65\pm    0.07$ & $   -5.28\pm    0.08$ & $  0.91\pm  0.30$\cr
  NGC~4291 & E$\cap$ &   28.6 &   10.272&
     6.3 &    9.271 &     0.81 &
$   -5.29\pm    0.03$ & $   -7.71\pm    0.03$ &
 $   -4.56\pm    0.02$ & $   -5.22\pm    0.03$ & $  0.65\pm  0.30$\cr
  NGC~4472 & E$\cap$ &   15.3 &   10.960&
     9.0 &    9.417 &     1.08 &
$   -5.36\pm    0.20$ & $   -7.79\pm    0.20$ &
 $   -4.43\pm    0.13$ & $   -5.01\pm    0.14$ & $  1.16\pm  0.28$\cr
  NGC~4473 & E$\cap$ &   15.8 &   10.252&
     5.1 &    8.533 &     0.21 &
$   -5.35\pm    0.14$ & $   -7.76\pm    0.15$ &
 $   -4.80\pm    0.02$ & $   -4.75\pm    0.15$ & $  0.52\pm  0.29$\cr
\noalign{\vskip3pt}
  NGC~4486 & E$\cap$ &   15.3 &   10.884&
    10.8 &    9.558 &     1.70 &
$   -5.67\pm    0.15$ & $   -8.10\pm    0.15$ &
 $   -4.17\pm    0.22$ & $   -4.75\pm    0.22$ & $  1.42\pm  0.31$\cr
 NGC~4486b & E$\cap$ &   15.3 &    8.960&
     3.6 &    8.963 &     2.23 &
$   -5.64\pm    0.18$ & $   -8.06\pm    0.19$ &
 $   -5.32\pm    0.26$ & $   -6.23\pm    0.37$ & $  0.68\pm  0.40$\cr
  NGC~4552 & E$\cap$ &   15.3 &   10.352&
     6.8 &    8.668 &     0.29 &
$   -4.88\pm    0.06$ & $   -7.30\pm    0.06$ &
 $   -4.91\pm    0.08$ & $   -5.57\pm    0.11$ & $  1.02\pm  0.34$\cr
  NGC~4564 & E$\setminus$ &   15.3 &    9.908&
     5.3 &    8.404 &     0.03 &
$   -4.26\pm    0.44$ & $   -4.51\pm    1.53$ &
 $   -4.25\pm    0.31$ & $   -4.20\pm    1.21$ & $ -0.30\pm  0.76$\cr
\noalign{\vskip3pt}
  NGC~4594 & S0$\setminus$ &    9.2 &   10.644&
     6.5 &    8.811 &     0.73 &
$   -5.26\pm    0.08$ & $   -7.68\pm    0.08$ &
 $   -4.67\pm    0.05$ & $   -5.31\pm    0.04$ & $  0.96\pm  0.38$\cr
  NGC~4621 & E$\setminus$ &   15.3 &   10.440&
     7.0 &    8.445 &     0.14 &
$   -4.26\pm    0.14$ & $   -6.66\pm    0.14$ &
 $   -4.05\pm    0.06$ & $   -5.21\pm    0.15$ & $  0.67\pm  0.46$\cr
  NGC~4636 & E$\cap$ &   15.3 &   10.600&
     8.1 &    8.356 &     0.28 &
$   -5.47\pm    0.10$ & $   -7.80\pm    0.08$ &
 $   -5.60\pm    0.07$ & $   -5.43\pm    0.14$ & $  1.04\pm  0.30$\cr
  NGC~4649 & E$\cap$ &   15.3 &   10.788&
     8.6 &    9.592 &     1.75 &
$   -5.49\pm    0.01$ & $   -7.91\pm    0.01$ &
 $   -4.21\pm    0.18$ & $   -4.80\pm    0.19$ & $  1.19\pm  0.26$\cr
\noalign{\vskip3pt}
  NGC~4660 & E$\setminus$ &   15.3 &    9.476&
     4.5 &    8.446 &     0.07 &
$   -3.81\pm    0.42$ & $   -5.05\pm    0.83$ &
 $   -3.85\pm    0.26$ & $   -4.63\pm    0.59$ & $ -0.13\pm  0.90$\cr
  NGC~4874 & E$\cap$ &   93.3 &   11.348&
     9.2 &   10.319 &     2.24 &
$   -6.20\pm    0.11$ & $   -8.64\pm    0.11$ &
 $   -4.00\pm    0.09$ & $   -4.59\pm    0.09$ & $  0.76\pm  0.20$\cr
  NGC~4889 & E$\cap$ &   93.3 &   11.276&
     6.4 &   10.429 &     2.49 &
$   -6.36\pm    0.10$ & $   -8.79\pm    0.10$ &
 $   -3.67\pm    0.07$ & $   -4.26\pm    0.07$ & $  0.61\pm  0.17$\cr
  NGC~6166 & E$\cap$ &  112.5 &   11.320&
     7.7 &   10.467 &     3.95 &
$   -6.65\pm    0.04$ & $   -9.09\pm    0.04$ &
 $   -4.14\pm    0.04$ & $   -4.74\pm    0.04$ & $  0.76\pm  0.21$\cr
\noalign{\vskip3pt}
  NGC~7768 & E$\cap$ &  103.1 &   11.104&
     6.9 &    9.933 &     0.87 &
$   -5.90\pm    0.07$ & $   -8.33\pm    0.06$ &
 $   -4.07\pm    0.08$ & $   -4.66\pm    0.08$ & $  0.33\pm  0.29$\cr
}\tabletext{
The second column gives the galaxy type: ``S0''=lenticular, ``S''=spiral
bulge, ``E''=elliptical; ``$\bigcap$'' = cored, ``$\setminus$'' = power
law (Lauer et al.\ 1995).  The distance $D$, luminosity $L_V$,
best-fit mass-to-light ratio $\Upsilon_V$ and black hole mass
$M_\bullet$ for each galaxy are taken from Paper~I
(which assumes $H_0=80{\rm\,km\,s^{-1}\,Mpc^{-1}}$).  $r_{\rm h}$ is
the radius of the sphere of influence of the BH.  $F^{\rm
lc}_\odot$ is the steady-state rate stars drift into the loss cone by
two-body relaxation (Section~3), neglecting the effects of
centrophilic orbits and assuming that all stars have solar mass and
radius.  $F^{\rm lc}_{\rm MF}$ is the more interesting visible
flaring rate, calculated using the stellar mass function described in
Appendix~A.  $F_\odot$ and $F_{\rm MF}$ are the rates obtained
when the effects of both two-body relaxation and of
centrophilic orbits (Section~4) are included.  The errors give the
uncertainties due to each galaxy's unknown inclination angle; 
the real uncertainties are much larger.
The last column lists the mean and standard deviation of the distribution
of the logarithm of the apocentre radii of the disrupted stars.
}
\endtable
\bye

